The Effect of Sparsity on $k$-Dominating Set and Related First-Order Graph Properties

We revisit $k$-Dominating Set, one of the first problems for which a tight $n^k-o(1)$ conditional lower bound (for $k\ge 3$), based on SETH, was shown (P\u{a}tra\c{s}cu and Williams, SODA 2007). However, the underlying reduction creates dense graphs, raising the question: how much does the sparsity of the graph affect its fine-grained complexity? We first settle the fine-grained complexity of $k$-Dominating Set in terms of both the number of nodes $n$ and number of edges $m$. Specifically, we show an $mn^{k-2-o(1)}$ lower bound based on SETH, for any dependence of $m$ on $n$. This is complemented by an $mn^{k-2+o(1)}$-time algorithm for all $k\ge 3$. For the $k=2$ case, we give a randomized algorithm that employs a Bloom-filter inspired hashing to improve the state of the art of $n^{\omega+o(1)}$ to $m^{\omega/2+o(1)}$. If $\omega=2$, this yields a conditionally tight bound for all $k\ge 2$. To study if $k$-Dominating Set is special in its sensitivity to sparsity, we consider a class of very related problems. The $k$-Dominating Set problem belongs to a type of first-order definable graph properties that we call monochromatic basic problems. These problems are the natural monochromatic variants of the basic problems that were proven complete for the class FOP of first-order definable properties (Gao, Impagliazzo, Kolokolova, and Williams, TALG 2019). We show that among these problems, $k$-Dominating Set is the only one whose fine-grained complexity decreases in sparse graphs. Only for the special case of reflexive properties, is there an additional basic problem that can be solved faster than $n^{k\pm o(1)}$ on sparse graphs. For the natural variant of distance-$r$ $k$-dominating set, we obtain a hardness of $n^{k-o(1)}$ under SETH for every $r\ge 2$ already on sparse graphs, which is tight for sufficiently large $k$.

==> chapters/partial-domination.tex <==
%auto-ignore
\section{Algorithms and Hardness of Partial Domination}
\begin{lemma}
    Let $G$ be a graph with maximal degree $\Delta$ and $k\geq 2$ a fixed constant.
    Then one can compute all the non-zero elements of the $k$-dimensional lookup table $B$, such that $B[v_1,\dots, v_k] = |N(v_1)\cap \dots \cap N(v_k)|$ in time $\bigO(m\Delta^{k-1})$.
\end{lemma}
\begin{proof}
    Iterate through all edges.
    For any edge $\{u,v\}$ go over all the $(k-1)$-element subsets $x_1,\dots, x_{k-1}$ of $N(v)\setminus \{u\}$ and increase the value of $B[u,x_1,\dots,x_{k-1}]$ (and all of their permutations) by $\frac{1}{k}$.
    Do the same for the other endpoint.

    To prove the correctness, let $x_1,\dots, x_k$ be arbitrary vertices and fix any vertex $v\in N(x_1)\cap \dots \cap N(x_k)$.
    We claim that for all the edges incident to $v$, we increase the value of $B[x_1,\dots, x_k]$ by exactly one.
    
    For all of the edges $\{v,x_1\},\dots, \{v,x_k\}$, we increase the value of $B[x_1,\dots, x_k]$ by $\frac{1}{k}$, hence in total we increase it by at least one.
    For the upper bound observe that if a value $B[x_1,\dots,x_k]$ is changed in an iteration, this iteration has to see an edge that contains at least one of the vertices $x_1,\dots, x_k$. 
    But since we are only considering the edges incident to $v$, we can observe that all the choices have been exhausted.

    Hence it follows directly that when the algorithm terminates, the value of $B[x_1,\dots, x_k]$ will be increased by exactly one for every vertex in $N(x_1)\cap \dots N(x_k)$ as desired.

    Time complexity of the algorithm is clearly at most $\bigO(m\Delta^{k-1}k!) = \bigO(m\Delta^{k-1})$
\end{proof}


\label{sec:partial-dom}


==> imports_template.tex <==
\usepackage[mathscr]{eucal}
\usepackage[fleqn]{amsmath}
\usepackage{amssymb,bbm,amsthm}
\usepackage{thm-restate,thmtools}
\usepackage{subcaption}
\usepackage[utf8]{inputenc}
\usepackage{graphicx}
\usepackage{hyperref}
\newcommand{\T}{\mathcal{T}}
\newcommand{\bigO}{\mathcal{O}}
\newcommand{\tww}{{\rm tww}(G)}
\newcommand{\G}{\mathcal{G}}
\usepackage{comment,color}
\usepackage{mathtools}
\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}
\usepackage{amsthm}
\usepackage{float}
\usepackage{cancel}
\usepackage[linesnumbered,boxed]{algorithm2e}
\usepackage[margin=1in, papersize={8.5in,11in}]{geometry}

\usepackage{enumitem}


\newcommand\mycommfont[1]{\footnotesize\ttfamily\textcolor{blue}{#1}}
\newcommand{\ksubset}{\genfrac{[}{]}{0pt}{}}
\newcommand*\xor{\oplus}
\newcommand{\F}{\mathbb{F}}

\SetCommentSty{mycommfont}
% \newtheorem{conjecture}{Conjecture}
% \newtheorem{exmp}{Example}

% \theoremstyle{definition}
% \newtheorem{definition}{Definition}
% \newtheorem{example}{Example}
% \theoremstyle{plain}
% \newtheorem{theorem}{Theorem}
% \newtheorem{assumption}{Assumption}
% \newtheorem*{claim}{Claim}
% \newtheorem{lemma}{Lemma}
% \newtheorem{observation}{Observation}
% \newtheorem{corollary}{Corollary}
% \newtheorem{proposition}{Proposition}

\declaretheorem[numberwithin=section]{theorem}
\declaretheorem[unnumbered, name=Theorem]{theorem*}
\declaretheorem[numberlike=theorem]{lemma}
\declaretheorem[numberlike=theorem,name=Lemma]{lem}
\declaretheorem[numberlike=theorem]{fact}
\declaretheorem[numberlike=theorem]{proposition}
\declaretheorem[numberlike=theorem,name=Proposition]{prop}
\declaretheorem[numberlike=theorem]{corollary}
\declaretheorem[numberlike=theorem,name=Corollary]{cor}
\declaretheorem[numberlike=theorem]{claim}
\declaretheorem[numberlike=theorem]{subclaim}
\declaretheorem[numberlike=theorem]{assumption}
\declaretheorem[numberlike=theorem]{observation}
\declaretheorem[numberlike=theorem]{invariant}
\declaretheorem[numberlike=theorem]{example}
\declaretheorem[numberlike=theorem]{remark}
\declaretheorem[numberlike=theorem, name=Definition]{definition}
\declaretheorem[unnumbered, name=Definition]{definition*}
\declaretheorem[numberlike=theorem, name=Conjecture]{conjecture}
\declaretheorem[unnumbered, name=Conjecture]{conjecture*}
\declaretheorem[numberlike=theorem, name=Hypothesis]{hypothesis}
\declaretheorem[unnumbered, name=Hypothesis]{hypothesis*}
\declaretheorem[numberlike=theorem,name=Open Question]{question}
\declaretheorem[numberlike=theorem,name=Problem]{problem}

\newcommand{\rem}[3]{\textcolor{blue}{\textsc{#1 #2:}}
  \textcolor{red}{\textsf{#3}}}
\newcommand{\marvin}[2][says]{\rem{Marvin}{#1}{#2}}
\newcommand{\mirza}[2][says]{\rem{Mirza}{#1}{#2}}
\newcommand{\nick}[2][says]{\rem{Nick}{#1}{#2}}

\newcommand{\tOh}{\tilde{\mathcal{O}}}

\newcommand{\FOP}[1]{$\mathrm{FOP}_k$}

\makeatletter
\renewcommand\paragraph{%
  \@startsection{paragraph}
    {4}
    {\z@}
    {3.25ex \@plus1ex \@minus.2ex}
    {-1em}
    {\normalfont\normalsize\bfseries\addperiod}}
\newcommand{\addperiod}[1]{#1\@addpunct{.}}
